Demoting Racial Bias in Hate Speech Detection

In current hate speech datasets, there exists a high correlation between annotators' perceptions of toxicity and signals of African American English (AAE). This bias in annotated training data and the tendency of machine learning models to amplify it cause AAE text to often be mislabeled as abusive/offensive/hate speech with a high false positive rate by current hate speech classifiers. In this paper, we use adversarial training to mitigate this bias, introducing a hate speech classifier that learns to detect toxic sentences while demoting confounds corresponding to AAE texts. Experimental results on a hate speech dataset and an AAE dataset suggest that our method is able to substantially reduce the false positive rate for AAE text while only minimally affecting the performance of hate speech classification.

==> acl2020-templates/abstract.tex <==
In the task of hate speech detection, there exists a high correlation between African American English (AAE) and annotators' perceptions of toxicity in current datasets. This bias in annotated training data and the tendency of machine learning models to amplify it cause AAE text to often be mislabeled as abusive/offensive/hate speech (high false positive rate) by current hate speech classifiers. Here, we use adversarial training to mitigate this bias. Experimental results on two hate speech datasets and one AAE dataset suggest that our method is able to reduce the false positive rate for AAE text without compromising the performance of hate speech classification.

==> acl2020-templates/intro.tex <==

\input{acl2020-templates/ex.tex}
The prevalence of toxic comments on social media and the mental toll on human moderators has generated much interest in automated systems for detecting hate speech and abusive language \cite{schmidt-wiegand-2017-survey, fortuna2018survey}, especially language that targets particular social groups \cite{silva2016analyzing, mondal2017measurement, mathew2019spread}. However, deploying these systems without careful consideration of social context can increase marginalization, bias, and exclusivity \cite{bender2018data,waseem2016hateful, davidson2017automated, founta2018large}.

Most data sets currently used to train hate speech classifiers were collected through crowd-sourced annotations \citep{davidson2017automated, founta2018large}, even though annotator biases exist since non-experts are more likely to label text as abusive than expert annotators \citep{waseem2016you}. \citet{sap2019risk} show how lack of social context in annotation tasks further increases the risk of annotator bias, which can in turn lead to the marginalization of racial minorities. More specifically, annotators are more likely to label comments as abusive if they are written in African American English (AAE). These comments are assumed to be incorrectly labelled, as annotators do not mark them as abusive if they are properly primed with dialect and race information. 

Classifiers trained on these biased annotations are more likely to incorrectly label AAE text as abusive than non-AAE text: the false positive rate (FPR) is higher for AAE text, which risks further suppressing an already marginalized community. According to \citet{sap2019risk}, the false positive rate for hate speech/abusive language of the AAE dialect can reach as high as 46\%.

\citet{sap2019risk} reveal two related issues in the task of hate speech classification: the first is biases in existing annotations and the second is model tendencies to absorb and even amplify these biases \cite{zhao2017men, DBLP:journals/corr/abs-1809-07842}.
While current data sets can be re-annotated, this process is time-consuming and expensive.
Furthermore, even with perfect annotations, current models may still learn and amplify spurious correlations between AAE and abusive language \cite{zhao2017men, DBLP:journals/corr/abs-1809-07842}.

% Such missing contexts may cause negative impacts on both the annotation process and the modeling process of hate speech detection. During the annotation process, without social contexts and enough background knowledge over hate speech, the annotators might be unaware of certain aspects that are crucial to determining whether a remark is a hate speech or not.

% Expert annotators outperform armature ones, with the latter being more likely to label items as hate speech \cite{waseem2016you} and causing misclassifications over the minority group. 

% \citet{sap2019risk} show that the annotators' insensitivity to English dialects leads to annotation bias where African American English markers (AAE) are highly correlated with a high level of toxicity, which is effectively mitigated through dialect and race priming.

% While re-annotating data can be extremely expensive, however, even without annotation bias, we are still faced with the issue that current models can easily pick up the racial bias in the data and unfortunately even amplify it \cite{zhao2017men, DBLP:journals/corr/abs-1809-07842}, while these biases are not inert or simply a reflection of data.

% To be more concrete, we show two example excerpted from \citet{founta2018large} and \citet{blodgett2016demographic} in \autoref{tab:example}, where an normal AAE tweet is mis-classified to be abusive language.

In this work, we present an adversarial approach to mitigating the risk of racial bias in hate speech classifiers, even when there might be annotation bias in the underlying training data.
In \Sref{sec:model}, we describe our methodology in general terms, as it can be useful in any text classification task that seeks to predict a target attribute (toxicity) without basing predictions on a protected attribute (AAE).
Although we aim at preserving the utility of classification models, our primary goal is not to improve the raw performance over predicting the target attribute (hate speech detection), but rather to reduce the influence of the protected attribute.


% We use adversarial training to reduce the effect of dialect (specifically AAE) on text representations learned by a hate speech classifier, which discourages the classifier from using dialectal information to make predictions.
In \Sref{sec:experiments} and \Sref{sec:results}, we evaluate how well our approach reduces the risk of racial bias in hate speech classification by measuring the FPR of AAE text, i.e., how often the model incorrectly labels AAE text as abusive.
%To quantitatively evaluate how biased a model is, we use false positive rate for hate speech of a group that is biased against (AAE) as a measure. 
We evaluate over two types of data: (1) datasets annotated for hate speech where we automatically infer language variety \cite{davidson2017automated, founta2018large} and (2) a dataset annotated for AAE language \cite{blodgett2016demographic}. Overall, our approach decreases the dialectal information encoded by the model, leading to a 1.1--~4.2 reduction in FPR for AAE text, without reducing performance on hate speech classification accuracy. 


% However, currently, the formulation of the hate speech detection task does not really take these factors into account - each data sample of commonly used datasets \cite{waseem2016hateful, davidson2017automated, founta2018large} usually comprises of a span of text and the its annotated label. Such contextual information is hard to acquire primarily due to a risk of a bleach of user privacy. 
 % In reality, determining what is a hate speech is still debatable as it might be affected by other contextual information such as the identity of the authors and recipients, co-occurring media objects \cite{schmidt2017survey}. 
 
%  Adversarial training is widely known for its success in learning disentangled representations from unwanted attributes, such as demographic and topical ones \cite{li-etal-2018-towards, elazar2018adversarial, kumar2019topics}. On top of the classification model, we augment the model by adding a discriminator responsible for predicting a binary label, whether the text is written in African American English or not. 

==> acl2020-templates/model.tex <==
Our goal is to train a model that can predict a target attribute (abusive or not abusive), but that does not base decisions off of a protected attribute (AAE dialect). In order to achieve this, we use an adversarial objective, which discourages the model from encoding information about the protected attribute. Adversarial training is widely known for successfully encouraging models to learn representations that are invariant to unwanted attributes, such as demographics and topics, though they rarely disentangle attributes completely \cite{li-etal-2018-towards, elazar2018adversarial, kumar2019topics,lample2018multipleattribute}.

%On top of the classification model, we augment the model by adding a discriminator responsible for predicting a binary label, whether the text is written in African American English or not.

\paragraph{Model Structure} Our demotion model consists of three parts: 1) 
An encoder $H$ that encodes the text into a high dimensional space; 2) A binary classifier $C$ that predicts the target attribute from the input text; 3) An adversary $D$ that predicts the protected attribute from the input text. The encoder is a single-layer bidirectional LSTM module with an attention mechanism. Both classifiers are two-layer MLPs with a tanh activation function. 

\paragraph{Training Procedure} Each data point in our training set is a triplet $\{(x_i, y_i, z_i); i \in 1 \dots N \}$, where $x_i$ is the input text, $y_i$ is the label for the target attribute and $z_i$ is label of the protected attribute. The $(x_i, y_i)$ tuples are used to train the classifier $C$, and the $(x_i, z_i)$ tuple is used to train the adversary $D$.

We adapt a two-phase training procedure from \citet{kumar2019topics}. In the first phase (pre-training), we use the standard supervised training objective to update encoder $H$ and classifier $C$:
\begin{gather}
    \min_{C, H} \sum_{i=1}^{N}  \mathcal{L}(C(H(x_i)), y_i)
    \label{eq:pretrain}
\end{gather}
After pre-training, the encoder should encode all relevant information that is useful for predicting the target attribute, including information predictive of the protected attribute.

In the second phase, starting from the best-performing checkpoint in the pre-training phase, we alternate training the adversary $D$ with \autoref{eq:tstep} and the other two models ($H$ and $C$) with \autoref{eq:cstep}:

\begin{align}
\begin{split}\label{eq:tstep}
      \min_D \frac{1}{N} \sum_{i=1}^{N} {}&  \mathcal{L}(D(H(x_i)), z_i)
\end{split}\\
\begin{split}\label{eq:cstep}
\min_{H, C}\frac{1}{N} \sum_{i=1}^{N} {}& \alpha \cdot \mathcal{L}(C(H(x_i)), y_i) + \\ 
& (1-\alpha) \cdot \mathcal{L}(D(H(x_i)), 0.5)
\end{split}
\end{align}

We first train the adversary to predict the protected attribute from the text representations outputted by the encoder.
We then train the encoder to ``fool'' the adversary by generating representations that will cause the adversary to output random guesses, rather than accurate predictions. At the same time, we train the classifier to predict the target attribute from the encoder output. 


Unlike prior work \citep{kumar2019topics}, we introduce a hyper-parameter $\alpha$, which controls the balance between the two loss terms in \autoref{eq:cstep}. 
We find that $\alpha$ is crucial for correctly training the model.


% update the encoder and the classifier with a weighted sum of a normal classification loss and a regularization loss.
%The classification loss is used to maintain properties needed for classification in text representations while adding the regularization loss meanwhile plays against the adversary to disable the encoder from encoding dialectal information.
  


==> acl2020-templates/stats.tex <==
\begin{table}[t]
\begin{tabular}{lll}
\toprule
  Dataset                                  & DWMW17 & FDCL18 \\ \midrule
AAE tweets                           & 13528  & 12415  \\
Negative AAE tweets & 12900  & 8812   \\ \midrule
Percentage                          & 95.36 \% & 70.98 \% \\
\bottomrule
\end{tabular}
\caption{Data statistics of offensive/abusive/Hateful (negative) tweets in AAE group.}
\label{tab:stats}
\end{table}
